Convergence rates of Kernel Conjugate Gradient for random design regression

We prove statistical rates of convergence for kernel-based least squares regression from i.i.d. data using a conjugate gradient algorithm, where regularization against overfitting is obtained by early stopping. This method is related to Kernel Partial Least Squares, a regression method that combines supervised dimensionality reduction with least squares projection. Following the setting introduced in earlier related literature, we study so-called "fast convergence rates" depending on the regularity of the target regression function (measured by a source condition in terms of the kernel integral operator) and on the effective dimensionality of the data mapped into the kernel space. We obtain upper bounds, essentially matching known minimax lower bounds, for the $\mathcal{L}^2$ (prediction) norm as well as for the stronger Hilbert norm, if the true regression function belongs to the reproducing kernel Hilbert space. If the latter assumption is not fulfilled, we obtain similar convergence rates for appropriate norms, provided additional unlabeled data are available.

==> macrogilles_main.tex <==
%Packages standard

\RequirePackage[isolatin]{inputenc}
\RequirePackage{comment}
\RequirePackage{graphicx}
\RequirePackage{amsmath,amsfonts}
\RequirePackage{color}
%Theoremes

\ifx \skiptheorems \thiscommandisnotdefinedtralala  
                 %teste si \skiptheorems est non-defini

\RequirePackage{amsthm}

\ifx \gillesfrench \thiscommandisnotdefinedtralala  

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{property}[theorem]{Property}
\newtheorem{example}[theorem]{Example}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\else

\newtheorem{theorem}{Théorème}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollaire}
\newtheorem{lemma}[theorem]{Lemme}


\theoremstyle{definition}
\newtheorem{definition}[theorem]{Définition}
\newtheorem{property}[theorem]{Propriété}
\newtheorem{example}[theorem]{Example}


\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remarque}

\fi
\fi

% Fontes

\newcommand{\mtc}{\mathcal}
\newcommand{\mbf}{\mathbf}

% Accents tildes over/underline etc

\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}

% Delimiteurs divers

\newcommand{\ind}[1]{{\mbf{1}\{#1\}}}
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\brac}[1]{\left[#1\right]}
\newcommand{\inner}[1]{\left\langle#1\right\rangle}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}

% Autres

\newcommand{\np}{_{_-}}
\newcommand{\pp}{_{_+}}
\newcommand{\defeq}{\stackrel{\cdot}{=}} % this is for
                                % definition-equal, not for number 2
                                % [This comment is (c) Gabór L. ]
\newcommand{\bydef}{:=}       % an alternative to defeq

% Operateurs proba

\newcommand{\var}[1]{{\rm Var}\brac{#1}}
\newcommand{\cov}[1]{{\rm Cov}\brac{#1}} 
\newcommand{\e}[1]{\mbe\brac{#1}}
\newcommand{\ee}[2]{\mbe_{#1}\brac{#2}}
\newcommand{\prob}[1]{\mbp\brac{#1}}
\newcommand{\probb}[2]{\mbp_{#1}\brac{#2}}


% Operateurs

\def\argmin{\mathop{\rm Arg\,Min}\limits}
\def\argmax{\mathop{\rm Arg\,Max}\limits}
\def\sgn{\mathop{\rm Sgn}\limits}
\def\tr{\mathop{\rm Tr}\limits}


% abbrev lettres grecques

\newcommand{\al}{\alpha}
\newcommand{\om}{\omega}
\newcommand{\eps}{\varepsilon}

% abbrev lettres mathcal

\def\cA{{\mtc{A}}}
\def\cB{{\mtc{B}}}
\def\cC{{\mtc{C}}}
\def\cD{{\mtc{D}}}
\def\cE{{\mtc{E}}}
\def\cF{{\mtc{F}}}
\def\cG{{\mtc{G}}}
\def\cH{{\mtc{H}}}
\def\cI{{\mtc{I}}}
\def\cK{{\mtc{K}}}
\def\cL{{\mtc{L}}}
\def\cM{{\mtc{M}}}
\def\cN{{\mtc{N}}}
\def\cO{{\mtc{O}}}
\def\cP{{\mtc{P}}}
\def\cQ{{\mtc{Q}}}
\def\cR{{\mtc{R}}}
\def\cS{{\mtc{S}}}
\def\cT{{\mtc{T}}}
\def\cU{{\mtc{U}}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

% abbrev lettres mathbb

\newcommand{\mbe}{\mathbb{E}}
\newcommand{\mbr}{\mathbb{R}}
\newcommand{\mbp}{\mathbb{P}}
\newcommand{\mbq}{\mathbb{Q}}
\newcommand{\mbi}{\mathbb{I}}
\newcommand{\mbn}{\mathbb{N}}
\newcommand{\mbz}{\mathbb{Z}}
\newcommand{\mbs}{\mathbb{S}}


% abbrev lettres en gras

\newcommand{\bA}{{\mbf{A}}}
\newcommand{\bD}{{\mbf{D}}}
\newcommand{\bG}{{\mbf{G}}}
\newcommand{\bI}{{\mbf{I}}}
\newcommand{\bW}{{\mbf{W}}}
\newcommand{\bX}{{\mbf{X}}}
\newcommand{\bY}{{\mbf{Y}}}
\newcommand{\bZ}{{\mbf{Z}}}


\newcommand{\bp}{{\mbf{p}}}
\newcommand{\bx}{{\mbf{x}}}

% frak

\newcommand{\fP}{{\mathfrak{P}}}
\newcommand{\fK}{{\mathfrak{K}}}

% TODO command

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% A command to put notes in a draft

\newcounter{nbdrafts}
\setcounter{nbdrafts}{0}
\makeatletter
\newcommand{\checknbdrafts}{
\ifnum \thenbdrafts > 0
\@latex@warning@no@line{**********************************************************************}
\@latex@warning@no@line{* The document contains \thenbdrafts \space draft note(s)}
\@latex@warning@no@line{**********************************************************************}
\fi}
\newcommand{\todo}[1]{\addtocounter{nbdrafts}{1}{\color{red} #1}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

